Video ReCap: Recursive Captioning of Hour-Long Videos

Most video captioning models are designed to process short video clips of few seconds and output text describing low-level visual concepts (e.g., objects, scenes, atomic actions). However, most real-world videos last for minutes or hours and have a complex hierarchical structure spanning different temporal granularities. We propose Video ReCap, a recursive video captioning model that can process video inputs of dramatically different lengths (from 1 second to 2 hours) and output video captions at multiple hierarchy levels. The recursive video-language architecture exploits the synergy between different video hierarchies and can process hour-long videos efficiently. We utilize a curriculum learning training scheme to learn the hierarchical structure of videos, starting from clip-level captions describing atomic actions, then focusing on segment-level descriptions, and concluding with generating summaries for hour-long videos. Furthermore, we introduce Ego4D-HCap dataset by augmenting Ego4D with 8,267 manually collected long-range video summaries. Our recursive model can flexibly generate captions at different hierarchy levels while also being useful for other complex video understanding tasks, such as VideoQA on EgoSchema. Data, code, and models are available at: https://sites.google.com/view/vidrecap

==> tables/charades.tex <==
\begin{table}[]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{cccc}
\toprule
Method              & Backbone & Features     & mAP           \\
\toprule
EgoVLP              & TSF-B    & Video        & 25.0          \\
EgoVLP-2            & TSF-B    & Video        & 26.2          \\
HierVL              & TSF-B    & Video        & 26.0          \\
LaViLa              & TSF-B    & Video        & 26.8          \\
LaViLa + HierVidCap & TSF-B    & Video + S. Sum. & \textbf{27.5} \\
% \midrule
% LaViLa              & TSF-L    & Video        & 28.9          \\
% LaViLa + HierVidCap & TSF-L    & Video + Sum. & \textbf{29.1}\\
\bottomrule
\end{tabular}
}
\caption{\textbf{Zero-Shot Action Recognition on CharadesEgo}}
\label{tab:charades}
\end{table}

==> tables/main_caption.tex <==
\begin{table*}[t]
\centering
% \resizebox{1\textwidth}{!}{%
\begin{tabular}{ccccccc}
Method     & Train Data           & Visual Encoder       & Text  Decoder        & CIDEr                & ROUGE-L              & METEOR               \\
BLIP2      & \multicolumn{1}{l}{} & VIT-G                & FT5-XL               & 8.1                  & 7.4                  & 12.7                 \\
LAVA       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
Lavila     & Ego4D                & TSF-B                & GPT2                 & 93.00                & 47.90                & 28.00                \\
HierVidCap & Ego4D                & TSF-B                & GPT2                 & \textbf{98.35}       & \textbf{48.77}       & \textbf{28.28}      
\end{tabular}
% }
\caption{\textbf{Main Results on Ego4D dataset.\mi{1. May be we can remove R3. 2. Add LAVA+GPT3.5. 3. Complete Segment and Video for BLIP2 and LAVA. 4. We can also Add HierVidCap-U and add train params. column.}}}
\label{tab:main caption}
\end{table*}

==> tables/main_results.tex <==
\begin{table*}[t]
\Large
\centering
\resizebox{1\textwidth}{!}{%
\begin{tabular}{c|cccc|ccccccccc}
\toprule
\multirow{2}{*}{Model}   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Visual\\ Encoder\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Text \\ Decoder\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Train\\ Params\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pseudo\\ Ann.\end{tabular}} & \multicolumn{3}{c}{Clip Caption}                 & \multicolumn{3}{c}{Segment Description}          & \multicolumn{3}{c}{Video Summary}                \\ \cline{6-14}    &                                                                           &                                                                          &                                                                         &                                                                        & C              & R              & M              & C              & R              & M              & C              & R              & M              \\ \toprule
\textbf{Zero-Shot}               &                                                                           &                                                                          &                                                                         &                                                                        &                &                &                &                &                &                &                &                &                \\
BLIP2~\cite{li2023blip}                    & VIT-G                                                                     & FT5-XL                                                                   & 0                                                                       & \xmark   & 8.1            & 7.4            & 12.7           & -              & -              & -              & -              & -              & -              \\
BLIP2~\cite{li2023blip} + GPT3.5~\cite{brown2020language}           & VIT-G                                                                     & GPT3.5                                                                   & 0                                                                       & \xmark                                                                      & -              & -              & -              & 5.68           & 16.87          & 13.47          & 11.13          & 22.41          & 12.10          \\
LaViLa~\cite{zhao2023learning} + GPT3.5~\cite{brown2020language}          & TSF-B                                                                     & GPT3.5                                                                   & 0                                                                       & \xmark                                                                      & -              & -              & -              & 5.79           & 19.77          & 13.45          & 12.16          & 24.49          & 12.48          \\ \midrule
\textbf{Finetuned}                &                                                                           &                                                                          &                                                                         &                                                                        &                &                &                &                &                &                &                &                &                \\
LaViLa~\cite{zhao2023learning} + GPT2~\cite{radford2019language}            & TSF-B                                                                     & GPT2                                                                     & 336M                                                                    & \xmark                                                                      & -              & -              & -              & 38.22          & 38.10          & 16.58          & 17.98          & 29.48          & 12.81          \\
LaViLa~\cite{zhao2023learning} + FLANT5~\cite{chung2022scaling}          & TSF-B                                                                     & FLANT5                                                                   & 586M                                                                    &   \xmark    & -              & -              & -              & 39.13          & 38.77          & 16.88          & 20.12          & 30.06          & 13.17          \\
LaViLa~\cite{zhao2023learning}                   & TSF-B                                                                     & GPT2                                                                     & 86M                                                                     & \xmark                                                                      & 88.56          & 47.64          & 28.03          & 24.63          & 33.31          & 15.30          & 6.54           & 23.97          & 10.95          \\
\model    & TSF-B                                                                     & GPT2                                                                     & 339M                                                                    & \xmark                                                                      & \textbf{98.35} & \textbf{48.77} & \textbf{28.28} & 41.74          & 39.04          & 18.21          & 28.06          & 32.27          & 14.26          \\
\model    & TSF-B                                                                     & GPT2                                                                     & 339M                                                                    & \cmark                                                                      & - & - & - & \textbf{46.88} & \textbf{39.73} & \textbf{18.55} & 29.34          & 32.64          & \textbf{14.45} \\
\model -U & TSF-B                                                                     & GPT2                                                                     & 113M                                                                    & \cmark                                                                      & 92.67          & 47.90          & 28.08          & 45.60          & 39.33          & 18.17          & \textbf{31.06} & \textbf{33.32} & 14.16          \\ \bottomrule
\end{tabular}
}
\caption{\textbf{Main Results on the \dataset\ dataset.} All results are evaluated in standard CIDEr (C), ROUGE-L (R) and METEOR (M) metrics. We observe several interesting trends. First, finetuned methods perform significantly better than the zero-shot baselines. Second, the \model\ model achieves the best results in video captioning across all three hierarchies, surpassing strong prior baselines such as \lavila~\cite{zhao2023learning}. Third, using LLM-generated pseudo annotations leads to a significant boost in performance. Lastly, the unified variant of the model produces competitive results while having a significantly smaller number of trainable parameters than our standard variant.}

%Second, the \model\ model stands out by achieving the best results in clip captioning, surpassing the previous leading method, \lavila~\cite{zhao2023learning}, by 9.79\% in CIDEr. Furthermore, our approach excels in segment description and video summary performance, outperforming the second-best model, \lavila~\cite{zhao2023learning} + FLANT5~\cite{chung2022scaling}, by 2.61\% and 7.94\% in CIDEr, respectively, while employing a substantially smaller number of trainable parameters.}
\label{tab:main results}
\end{table*}









==> tables/recursive.tex <==
\begin{table}[t]
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Recursive\\ Input\end{tabular}} & \multicolumn{3}{c|}{Segment Description}             & \multicolumn{3}{c}{Video Summary}                \\ \cline{2-7} & C              & R              & M              & C              & R              & M              \\ \toprule
\xmark                                                                          & 40.17          & 38.65          & 17.59          & 25.64          & 29.61          & 13.57          \\
\cmark                                                                          & \textbf{41.74} & \textbf{39.04} & \textbf{18.21} & \textbf{28.06} & \textbf{32.27} & \textbf{14.26} \\ \bottomrule
\end{tabular}
}
\vspace{-0.3cm}
\caption{\textbf{Inportance of Recursive Inputs.} A non-recursive variant of our model performs worse in segment description and video summary generation (-1.57\%  and -2.42\% in CIDEr).\vspace{-0.3cm}}
\label{tab: recursive}
\end{table}
